Some bijective correspondences involving domino tableaux

We define a number of new combinatorial operations on skew semistandard domino tableaux, which together with constructions introduced earlier by C. Carre and B. Leclerc, define an elegant structure on the set of these tableaux, that closely parallels the structure defined in [math.CO/9908099] for ordinary skew semistandard tableaux, that is related to the Littlewood-Richardson rule. These operations are: (1) a bijection between semistandard domino tableaux and certain pairs of ordinary tableaux of the same weight that together fill the same shape; (2) a weight preserving transformation of domino tableaux to ordinary tableaux of a related shape (the correspondence involves 2-quotients) with the property that Yamanouchi domino tableaux correspond precisely to Littlewood-Richardson tableaux; (3) a correspondence between Yamanouchi domino tableaux of shape $\lambda$ and weight $\mu$ and Yamanouchi domino tableaux of shape $\mu'$ and weight $\lambda$, where $\mu'$ is $\mu$ scaled by a factor 2. The property at the heart of the structure so defined is that operations (1) and (2) commute with the coplactic operations (implicitly) defined by Carre and Leclerc. (1) elucidates their bijection analogous to that of Robinson (a.k.a. the Robinson-Schensted correspondence), while the operation of moving chains in domino tableaux underlying (2) is very similar to jeu de taquin.

==> marxmax.tex <==
% Protection

\ifx\macrosloaded\relax  \endinput \else \let\macrosloaded\relax \fi
\ifx\formloaded\undefined \input form \fi

\catcode`@=11

% TeXnical tricks

\def\letnext{\let\next= }
\def\defnext{\def\next}   % Not \outer, in case \next is.

\newif\ifamstex {\defnext{AmS-TeX} \ifx\fmtname\next \global\amstextrue \fi}

\def\reset#1{\global#1=0 }
\def\useouter #1 {\begingroup
                  \expandafter\let\csname#1\endcsname=\relax % not outer
                  \afterassignment\endgroup\global}
\def\?#1\then#2\else#3\fi{#1\defnext{#2}\else\defnext{#3}\fi \next}
\newif\ifnot
\newif\ifnomessage \nomessagetrue % used to suppress expansions in \message
\let\domessage=\message \def\message#1{{\nomessagefalse\domessage{#1}}}

% File handling

\newif\iftoc 
\def\writetoc{\write\tocfile}\def\tocfile{-1 }
\useouter newwrite
\def\opentoc{\newwrite\tocfile\openout\tocfile=\jobname.toc }
\edef\tocheader{\string\NotocSection\space Table of contents.
  \string\noindent\string\medskip}
\def\maketoc{\opentoc\writetoc{\tocheader}\toctrue}

\def\str#1{\string#1 }
% The following prohibits expansion between $..$,
% but there shouldn't be any groups there.
{\catcode`@=3 % weird math shifts, cannot occur in math mode
 \gdef\passord#1$#2\end{#1\ifx@#2@\else\getmath#2\end\fi}
 \gdef\getmath#1${$\noex#1\endmath$\passord}
 \gdef\noex#1\endmath{\ifx@#1@\else\donoex#1\endmath\fi}
 \gdef\donoex#1{\noexpand#1\noex}
 \gdef\nomathexp#1{\passord#1$\end}
}

\iffalse$\fi % to get emacs' font-lock adrift again

\def\putmark#1{\mark
  {\count1=\the\secno \count2=\the\subsecno \count3=\the\proclno
   \marktoks={\ignorespaces\setchap\space#1}}}% set counters, running head
\def\setchap{\ifnum\secno<0 Appendix \lastlabel.\else\lastlabel\fi}
\def\puttoc#1{\toks0={\nomathexp{#1} \str\onpage\folio.}\edef\next
                      {{\str\tocitem \lastlabel=\the\toks0}}\writetoc\next}
\def\setmark#1{\putmark{#1}\puttoc{#1}}

\output=
{\everyhbox{}% don't interfere into output routine
 \firstmark \headline={\tenit \ifodd\pageno\hfill\fi \the\marktoks \hfil }
 \let~\relax % ~ shouldn't be expanded in index file, and doesn't occur in:
 \plainoutput
}

\newwrite\labfile
\def\tolab{\write\labfile}
\def\writelab{\openout\labfile=\jobname.lab
              \global\let\writelab=\tolab \tolab}
\def\chklab#1\lastlabel#2.{\def\next{#2}\ifx\next\empty}% if #1/=\lastlabel
\def\deflab#1{\chklab#1\lastlabel.\writelab{\string\def\string#1{#1}}\fi}
\def\savecount#1{\writelab{#1=\number#1}}
\toks0={\savecount\secno\savecount\subsecno\savecount\proclno
        \savecount\eqnumber
        \savecount\pageno\writelab{\string\advancepageno}}
\toks2=\expandafter{\bye}
\edef\bye{\the\toks0 \the\toks2}


\newwrite\indexfile
\def\toindex{\write\indexfile}
\def\writeindex{\openout\indexfile=\jobname.inx
                \global\let\writeindex=\toindex \toindex}
\def\inx#1{\writeindex{\nomathexp{#1} @\folio.}}
\def\index#1{\inx{#1}#1}
\def\closeindex{\vfil\eject % Ensure final entries are written
                \ifx\writeindex\toindex \immediate\closeout\indexfile \fi}

% Layout style

\font\boldit=cmbxti10 % for subsection headings
\font\ssq=cmssq8 \font\ssqi=cmssqi8 % for quotations

\newcount\secno \newcount\subsecno \newcount\proclno \newcount\itemno
\reset\secno \reset\subsecno \reset\proclno \reset\itemno
\newdimen\itemindent \itemindent=\parindent % the default, but changable
\newtoks\marktoks

\let\Sec\S % Section mark
\useouter beginsection
 \outer\def\newsection #1.
  {\ifnewsec \endgroup \fi % previous (sub)section might be empty
   \global\advance\secno by 1
   \ifnum-1<\subsecno \reset\subsecno \fi % <0 means no subsections used
   \reset\proclno
   \edef\lastlabel{\number\secno}%
   {\parskip0pt\beginsection\ifnomessage\Sec\fi\lastlabel. #1.\par
    \par}% immediately terminate the paragraph started by \beginsection
   \setmark{#1}% this mark follows the non-breakable space below the title
   \startsec % this replaces the indent-defeating code of \beginsection
  }
\def\subsection #1.
  {\secbigbreak
   \global\advance\subsecno by 1 \reset\proclno
   \edef\lastlabel{\number\secno.\number\subsecno}%
    \leftline{\bf\lastlabel.\enspace
              \defnext{#1}\ifx\next\empty\else \boldit#1.\fi}\setmark{#1}%
    \nobreak\smallskip\startsec}
\useouter beginsection
 \outer\def\Appendix #1.
  {\ifnum\secno>0 \startapx\fi
   \global\advance\secno by -1 \reset\subsecno \reset\proclno
   \edef\lastlabel
    {\ifcase -\secno \or A\or B\or C\or D\or E\or F\or G\or H\or I\or J\fi}%
   {\parskip0pt\beginsection Appendix \lastlabel. #1.\par\par}%
   \setmark{#1}\startsec}
\def\startapx{\ifx\writetoc\totoc\totoc{\str\Appendices}\fi \secno=0 }
\useouter beginsection
 \outer\def\Supplement #1.
  {\let\lastlabel=\empty
   \global\ifnum\secno<0 \secno=1000 \else\advance\secno by 1 \fi
   \beginsection #1.\par\par\setmark{#1}\startsec}
\useouter beginsection
 \outer\def\NotocSection #1.
  {\let\lastlabel=\empty \reset\secno
   \beginsection #1.\par\par\putmark{#1}\startsec}

\newif\ifnewsec % communication with proclaim etc.
\def\startsec
  {\begingroup \newsectrue\parskip0pt\parindent0pt \everypar{\endgroup}}
\def\secbigbreak
  {\ifnewsec \endgroup
     \ifdim\lastskip<\bigskipamount \removelastskip\bigskip \fi % no penalty
   \else \bigbreak
   \fi}
\def\secmedbreak
  {\ifnewsec \endgroup
     \ifdim\lastskip<\medskipamount \removelastskip\medskip \fi % no penalty
   \else \medbreak
   \fi}
\def\labelsec#1{\global\let#1=\lastlabel \deflab#1\nobreak}% prolong nobreak

% for \startsec to work properly, a paragraph should not begin with `{text}'
% here we fix those macros that do such a thing. In the meantime we deactivate
% the accents within messages, so that only the base character will appear

{\let\x=\expandafter
 % in the following macro #1 is the \cs to be redefined; \next is defined to
 % do the redefinition, which it achieves using the old expansion passed to it
 % as an argument; after defining \next, it is called with the expansion of #1
 \def~#1{\defnext##1{\gdef#1{\ifnomessage\leavevmode##1\fi}}\x\next\x{#1}}
 ~\copyright
 % the following is similar, but now \cs itself takes one argument. When
 % passing the 'expansion' of \cs, that argument is given as '#1', which will
 % capture the formal argument of \cs in the redefinition within \next
 \def~#1{\defnext##1{\gdef#1####1{\ifnomessage\leavevmode##1\else####1\fi}}%
         \x\next\x{#1{##1}}}
 ~\` ~\' ~\v ~\^^_ ~\u ~\^^S ~\^ ~\^^D ~\. ~\H ~\~ ~\" 
 \ifamstex ~\B \else ~\= ~\t \fi
}


\def\quotation
{\begingroup\everypar{}\parfillskip=0pt
 \leftskip=0pt plus \hsize \def\par{\ifhmode\/\endgraf\nobreak\fi}\obeylines
 \let\it=\ssq\let\rm=\ssqi\rm % switch roman and italic
 \baselineskip=10pt\parskip=0pt
 \def\author##1, ##2.{\vskip2pt\it ##1, \rm ##2\par\smallskip\endgroup}
}

\newcount\eqnumber \eqnumber=0
\def\neqn(#1#2){\global\advance\eqnumber by 1
                (\ifcat a\noexpand#1%
                        \errmessage{Incorrect label #1#2}\number\eqnumber
                 \else\xdef#1{\number\eqnumber}\deflab#1%
                      #1\fam\z@#2% #2 is possible tail, like "a,b"
                 \fi)}
\def\label{\ifinner\else \eqno \fi \neqn}
\def\nn{\label(\lastlabel)}
\newcount\acc
\def\add#1#2{\acc=#1\advance\acc#2\relax\number\acc}

\def\heading "#1"{\smallbreak\noindent{\sl #1}.\quad\ignorespaces}

\let\proclaim=\relax
\ifamstex
% kludge needed because \endtopmatter sets \proclaim to \innerproclaim@ (again)
\let\amsproclaim=\innerproclaim@
\def\innerproclaim@#1. #2#3\par
  {\secmedbreak \global\advance\proclno by 1 \reset\itemno
   \edef\lastlabel{\number\secno\ifnum-1<\subsecno.\number\subsecno
                                \fi.\number\proclno}
   {\interlinepenalty=300 \parskip=0pt\def\par{\endgraf\penalty200 }% (item)
    \noindent % Emit \baselineskip & \parskip glue BEFORE doing \deflab
    \nottrue % here this means: no label to define
    \if\let\noexpand#2\ifx\undefined#2\notfalse\fi\fi% Is #2 undefined \cs?
    \ifnot\amsproclaim{\lastlabel.\enspace#1}#2#3\innerendproclaim@
    \else\global\let#2\lastlabel \deflab#2%
      \amsproclaim{\lastlabel.\enspace#1}#3\innerendproclaim@
    \fi
   }}
\else
\outer\def\proclaim#1. #2#3\par
  {\secmedbreak \global\advance\proclno by 1 \reset\itemno
   \edef\lastlabel{\number\secno\ifnum-1<\subsecno.\number\subsecno
                                \fi.\number\proclno}
   {\interlinepenalty=300 \parskip=0pt\def\par{\endgraf\penalty200 }% (item)
    \noindent % Emit \baselineskip & \parskip glue BEFORE doing \deflab
    \if\let\noexpand#2% Is #2 a control sequence?
     \ifx\undefined#2% don't redefine a control sequence
      \global\let#2\lastlabel \deflab#2\letnext\ignorespaces
     \else\defnext{#2}\fi
    \else\defnext{#2}\fi
    \bf\lastlabel.\enspace#1.\enspace \sl\next#3\endgraf
    }%
   \ifdim \lastskip<\medskipamount \removelastskip\penalty55\medskip \fi
   }
\fi

\def\dueto#1.{\unskip~[#1].}

\def\newpar{\ifhmode\par\fi{\parskip0pt\noindent}}% no extra vertical space
\def\enditem{\newpar\reset\itemno}
\def\item{\doindent\itemindent}
\def\itemitem{\doindent{2\itemindent}}
\def\doindent#1#2{\newpar
  \hangindent#1\hangafter0 \llap{#2\enspace}\ignorespaces}

\def\statitemnr#1{(\number#1)}
\def\statitem{\global\advance\itemno by 1 \item{\statitemnr\itemno}}
\def\eqitemnr#1{(\romannumeral#1)}
\def\eqitem{\global\advance\itemno by 1 \item{\eqitemnr\itemno}}
\def\defitemnr#1{\count@=#1\advance\count@96\char\count@}
\def\defitem{\global\advance\itemno by 1 \item{\defitemnr\itemno.}}

\def\proof{\heading "Proof"} \def\proofof#1{\heading "Proof of #1"}
\def\QED{\dimen0=.5em\advance\dimen0\wd\QEDbox\advance\dimen0.4pt
         \unskip\kern\dimen0\vadjust{\vskip-\baselineskip}\unhcopy\tightbox
         \copy\QEDbox{\pretolerance=1000\parfillskip=0.4pt\smallbreak}}
\def\QEDQED{\unskip\nobreak\enskip\kern\wd\QEDbox
            {\setbox\QEDbox=\hbox{\copy\QEDbox\enspace\copy\QEDbox}\QED}}

\def\emph#1{{\it #1}\futurelet\next\doitcor}
\def\newterm#1{{\sl\index{#1}}\futurelet\next\doitcor}
\def\foreign#1{{\sl #1}\futurelet\next\doitcor}
\def\doitcor{\if.\next\else\if,\next\else\/\fi\fi}
\def\needfil{\penalty-100\vfil\penalty1500\vfilneg}% raggedbottom, if needed
\def\bigdisplay{\ifmmode \errmessage{Display begun in math mode.}
                \else\ifhmode\unskip\vadjust{\needfil}%
                     \else\needfil\noindent\fi$$\fi}
\def\frame#1{\leavevmode\hbox{\vrule\vtop{\vbox{\hrule\kern2pt
     \hbox{\strut\kern2pt#1\kern2pt}}\kern2pt\hrule}\vrule}} % framed box
\def\clap#1{\hbox to 0pt {\hss#1\hss}}

\def\setbaselineskip{\par\afterassignment\setbskip\skip0 =}
\def\setbskip{\null\baselineskip=\skip0 \vskip-\baselineskip}
\def\forceeven{\eject\ifodd\pageno \null\mark{\marktoks{}}\vfil\eject \fi}
\def\forceodd{\eject\ifodd\pageno\else\null\mark{\marktoks{}}\vfil\eject\fi}
\def\topglue{\eject\afterassignment\topglu\skip0 }
\def\topglu{\hrule height0pt\vskip\skip0\vskip-\topskip
     \dimen0=\baselineskip\advance\dimen0-\topskip \prevdepth=\dimen0 }
\def\endraggedbottom{\par\penalty9999 % allow overfull page to go
  \normalbottom{\output={\unvbox255\penalty0 }\eject}}
% output routine resets topskip glue

\def\qdef#1{\?\ifx #1\undefined \then \def #1%
              \else \toks0={#1}\afterassignment\chkdef\def\next
              \fi}
\def\qqdef#1{%
\?\ifx #1\undefined
  \then \message{Patching definition:\string#1.}\let\Qdef=\qdef\def#1%
  \else \toks0={#1}\afterassignment\chkdef\def\next
  \fi}
\let\Qdef=\qqdef
\def\chkdef{\expandafter\let\expandafter\curcs\the\toks0 % space is crucial!
  \ifx\next\curcs\else
  \message{Altered definition:\the\toks0= \meaning\next,
                              should have been \meaning\curcs.}\fi}
\ifamstex
\def\mathtext#1{\quad\hbox{#1}\quad}
\def\mathttext#1{\qquad\hbox{#1}\qquad}
\def\mathtex#{\quad\hbox}
\def\mathttex#{\qquad\hbox}
\else
\def\text#1{\quad\hbox{#1}\quad} \def\ttext#1{\qquad\hbox{#1}\qquad}
\def\tex#{\quad\hbox}            \def\ttex#{\qquad\hbox}
\fi

\def\calign #1{\null\,\vcenter{\openup1\jot
     \ialign{\strut\hfil$\displaystyle##$\hfil\cr#1\crcr}}\,}

% Symbols

\newcount\t@
\def\mathdef #1=#2 #3%
{\count@=\z@
 {\def\t{#2}\nottrue
  \loop \xdef\next{\ifcase \count@
    Ord\or Op\or Bin\or Rel\or Open\or Close\or Punct\or VarFam\else #2\fi}%
    \ifx \next\t \notfalse \fi
  \ifnot \global\advance\count@ by 1 \repeat
 }\multiply\count@"1000
 \t@=\expandafter
 \ifx\expandafter\delimiter#3\divide\t@"1000 \nottrue
 \else
   \ifcat \alpha#3#3\nottrue
   \else \mathcode`#3 \ifnum\t@<"7000 \nottrue \else \notfalse \fi
   \fi
 \fi
 \advance\count@\t@
 \ifnot \divide\t@"1000 \multiply\t@"1000 \advance\count@-\t@
   \mathchardef#1=\count@
 \else \divide\t@"100 \multiply\t@"100 \advance\count@-\t@
   \def\next{#1}\afterassignment\mathd@f \t@=
 \fi
}
\def\mathd@f
{\multiply\t@"100 \advance\count@\t@ \expandafter\mathchardef\next=\count@}
\def\mathorddef #1={\mathdef #1=Ord }

\ifamstex \let\boldmath=\bold \let\romath=\roman
\else \def\boldmath#1{{\fam\bffam#1}} \def\romath#1{{\fam\z@#1}}
\fi

\mathorddef\N=N\bffam
\mathorddef\Z=Z\bffam
\mathorddef\Q=Q\bffam
\mathorddef\R=R\bffam
\mathorddef\C=C\bffam
\mathorddef\P=P\bffam
\def\Np{\N_{>0}}
\mathorddef\1=1\bffam
\mathorddef\2=2\bffam
\mathorddef\ii=i\bffam % imaginary unit
\mathorddef\\=\lambda
\mathdef\:=Punct :
\let\Id=\1
\mathorddef\Sym=S\bffam % symmetric group

\def\opdef#1{\def#1{\mathop\romath{\escapechar\m@ne\string#1}\nolimits}}
\def\altopdef#1#2{\def#1{\mathop\romath{#2}\nolimits}}
\def\li(#1#2..#3){%
  #1_{#2},\penalty\binoppenalty\ldots,\penalty\binoppenalty#1_{#3}}
\def\lix(#1#2.#3.#4){%
  #1_{#2},\penalty\binoppenalty\ldots,\widehat{#1_{#3}},\penalty\binoppenalty
  \ldots,#1_{#4}}
\def\fold#1(#2#3..#4){#2_{#3}#1\cdots#1#2_{#4}}
\def\foldx#1(#2#3.#4.#5){#2_{#3}#1\cdots#1\widehat{#2_{#4}}#1\cdots#1#2_{#5}}
\def\({\bigl(}\def\){\bigr)}
\def\inv{^{-1}}
\def\<#1>{{\langle #1\rangle}}
\let\oslash=\o \def\o{^\circ} \def\p{^\perp}

\def\defeq{\buildrel\topsmash{\romath{def}}\over =}
\mathdef\orbit=Bin \backslash
\let\union=\cup % used to be \mathdef\union=Rel \cup
                      \let\Union=\bigcup
\let\thru=\cap        \let\Thru=\bigcap
\let\disju=\amalg     \let\Disju=\coprod
\let\tensor=\otimes   \let\Tensor=\bigotimes
\let\directsum=\oplus \let\Directsum=\bigoplus
\let\implies=\Rightarrow
\let\act=\cdot
\let\after=\circ % function composition
\let\eps=\varepsilon
\def\setof#1:#2\endset{{\{\,#1\mid#2\,\}}}
\def\Setof#1:#2\endset{\left\{\,#1\,\,\vrule\,\,#2\,\right\}}
\let\isom=\cong \let\cong=\equiv \let\equiv=\sim % correct wrong names
\def\isomto{\buildrel\equiv\over\rightarrow}
\def\otmosi{\buildrel\equiv\over\leftarrow}
\let\ssubset=\subset \let\subset=\subseteq
\let\ssupset=\supset \let\supset=\supseteq
\let\baraccent=\= \def\={\relax\?\ifmmode\then\approx\else\baraccent\fi}

\opdef\sg \opdef\Ker\opdef\Im \opdef\Aut \opdef\End \opdef\rk
\altopdef\kar{char}
\def\Card#1{\##1}

% Standard abbrev.'s

\def\mo.{morphism}
\def\iso.{iso\mo.}
\def\cor.{correspond}
\def\de.{definition}
\def\De.{Definition}
\def\lcit{loc.\thinspace cit.}

% Boxes

\def\topsmash#1{{\def\finsm@sh{\ht\z@\z@ \box\z@}\smash{#1}}}
\def\botsmash#1{{\def\finsm@sh{\dp\z@\z@ \box\z@}\smash{#1}}}


\newbox\tightbox % for "tight" breaks
\setbox\tightbox=
\hbox{\penalty -200               \skip0 = 0pt plus 0.05 \hsize
      \hskip \skip0 \penalty    0 
      \hskip \skip0 \penalty  200 \skip0 = .1\hsize
      \hskip \skip0 \penalty  283 
      \hskip \skip0 \penalty  346
      \hskip \skip0 \penalty  400
      \hskip \skip0 \penalty  447 
      \hskip \skip0 \penalty  490
      \hskip \skip0 \penalty  529
      \hskip \skip0 \penalty  567 
      \hskip \skip0 \penalty  600
      \hskip \skip0 \penalty  632
      \hskip 2\hsize % make it an offer TeX can't refuse
      \vadjust{}\hfil} % warning if you change \hsize do it FIRST. 
\newbox\QEDbox
\setbox\QEDbox=\hbox
{\kern-0.2pt\vrule height 6pt \kern-0.4pt % backspace
 \vbox to 6pt
  {\kern -0.2pt
   \hbox to 6.4pt{\hrulefill\kern-0.2pt\vrule}\vfil
   \hrule width 6.2pt
   \kern -0.2pt}%
 \kern-0.4pt \vbox to 6pt{\leaders\vrule\vfil\kern-0.2pt}\kern-0.2pt
}

% Nine point type (for footnotes and references); math sizes 9--7--5 pt

\ifx\ninept\undefined % don't overwrite more sophisticated \ninept macros

\font\ninerm=cmr9 \font\nineit=cmti9 \font\ninebf=cmbx9 \font\ninesl=cmsl9
\font\ninett=cmtt9 \font\ninei=cmmi9 \font\ninesy=cmsy9
\skewchar\ninei='177 \skewchar\ninesy='60

\def\ninept
{\def\rm{\fam0\ninerm}\def\it{\fam\itfam\nineit}\def\bf{\fam\bffam\ninebf}%
 \def\sl{\fam\slfam\ninesl}\def\tt{\fam\ttfam\ninett}\rm
 \textfont0\ninerm \textfont1\ninei \textfont2=\ninesy
 \textfont\itfam\nineit \textfont\slfam\ninesl
 \textfont\bffam\ninebf \textfont\ttfam\ninett
 \normalbaselineskip=11pt \normalbaselines
 \setbox\strutbox=\hbox{\vrule height 8 pt depth 3 pt width 0 pt}%
}

\fi

\def\caps#1{{\ninept #1}}

\ifamstex
\let\amsfootnote=\footnote
\def\footnote#1{\amsfootnote"#1"}
\else
% redefine footnotes to be in 9pt type and independent of context settings
\def\vfootnote#1%
{\insert\footins\bgroup \ninept
 \interlinepenalty=\interfootnotelinepenalty
 \splittopskip=\ht\strutbox % determines top baselines of broken footnotes
 \splitmaxdepth=\dp\strutbox % likewise for bottom lines
 \floatingpenalty=20000 % please don't break footnotes, if possible
 \leftskip=1pc \rightskip=1pc \spaceskip=0pt \xspaceskip=0pt
 \parindent=0pt \parskip=3pt minus 1pt \parfillskip=0pt plus 1 fil
 \textindent{#1}\footstrut\futurelet\next\f@@t
}
\fi

% References

\catcode`_=11 % control sequence names with this letter are private

\newif\ifamsrefs % whether AMS style refernece syntax is used

\ifamstex
\let\amsref=\ref
\let\amsendref=\endref
\let\amspubl=\publ
\let\amsinbook=\inbook
\let\amskey=\key
\let\amsed=\ed \let\amseds=\eds
\let\amsvol=\vol
\let\amspages=\pages
\fi

\def\label_#1#2{\expandafter\xdef \csname#1.\endcsname{#2}}
\def\ref#1{\ref_#1,,,.}
\def\ref_#1,#2,,#3.{\expandafter\ref_lab\csname#1.\endcsname{#3#2}}
\def\ref_lab#1#2{\ifx #1\relax \errmessage{Reference to undefined label}%
                 \else [#1#2]\fi
                }

\newdimen\refindent
\refindent=36pt

\def\init_refs % For initialising reference labels at start of article
{\begingroup\setbox0=\vbox\bgroup \hbadness 10000 \hfuzz=\maxdimen
 \def\chapter ##1\par{}% avoid problems with chapter number and tocfile
 \def\endrefs{\egroup\egroup\endgroup\endinput}% end \beginrefs & \init_refs
 \ifamsrefs
 \else
  \def\endref{\iffalse{\fi}\ifx\the_key\undefined\else
     \label_{\expandafter\strip_space\the_key _}%
	    {\expandafter\strip_space\the_mark _}\fi
     \endgroup}%
 \fi
}
\def\strip_space #1 _{#1}

\def\readrefs{\init_refs \input \jobname.ref }

\useouter amsref \def\ams_start\key #1 \ident#2%
{\label_{#2}{#1}\amsref\amskey{#1}%
}
\outer\def\beginrefs{\noindent\par % fire up \everypar
 \ifamsrefs
  \bgroup \let\ref=\ams_start
  \let\publ=\amspubl \let\inbook=\amsinbook \let\key=\amskey
  \let\ed=\amsed \let\vol=\amsvol \let\pages=\amspages
 \else
  \bgroup \ninept
  \frenchspacing\tolerance=900
  \let\ref=\_ref \let\author=\_auth \let\title=\_tit
  \let\vol=\_vol \let\year=\_year
 \fi
}

\outer\def\endrefs{\egroup\smallbreak}

\def\ref_item#1{\iffalse{\fi}% must have an unbalanced explicit brace here
  \ifx#1\undefined \else
    \errmessage{Multiple definition of \string#1 within reference}\fi
  \edef#1{\iffalse}\fi % must be \edef to activate keywords (like \title)
}


\def\_ref{\begingroup
  \def\par{\endref\par}\def\ref{\endref\ref}\edef\the_mark{\iffalse}\fi}
\def\_auth{\ref_item\the_author}
\def\_tit{\ref_item\the_title}
\def\key{\ref_item\the_key}
\def\series{\ref_item\the_series}
\def\publ{\ref_item\the_publ}
\def\ISBN{\ref_item\the_ISBN}
\def\journal{\ref_item\the_journal}
\def\_vol{\ref_item\the_vol}
\def\_year{\ref_item\the_year}
\def\pages{\ref_item\the_pages\range_}
\def\npages{\ref_item\the_pages\amount_}
\def\idno{\ref_item\the_idno}
\def\inbook{\ref_item\the_inbook}
\def\ed{\ref_item\the_ed}
\def\report{\ref_item\the_report}
\def\endnote{\ref_item\the_endnote}

\def\range_{\noexpand\range_}   % these cancel the \edef in \ref_item
\def\amount_{\noexpand\amount_}
\def\do_amount{{\aftergroup\do_pp\aftergroup}}
\def\do_pp{~pp}
\def\expl_pp{\def\range_{pp.~}\let\amount_=\do_amount} % if `pp.' is desired
\def\impl_pp{\let\range_\empty\let\amount_=\do_amount} % if `pp.' not desired

\def\q_plur#1{\expandafter\q_s#1,_}\def\q_s#1,#2_{\ifx _#2_\else s\fi}

\def\_pages{\expandafter\pages_\the_pages\unskip---_}
\def\pages_#1-#2#3-#4_{#1\ifx _#4_\else\if -#2--#3\else --#2#3\fi\fi}

\ifamstex

\def\_opt#1#2{\ifx#1\undefined\else#2\fi}
\def\opt_pages{\_opt\the_pages{\amspages\expandafter\pages_\the_pages---_}}

\def\endref{\ifamsrefs \amsendref \else \ams_convert \fi}

\useouter amsref \def\ams_convert
{\iffalse{\fi}\let\par\endgraf
 \amsref \amskey\the_mark \by\the_author
 \ifx\the_inbook\undefined
   \ifx\the_journal\undefined
     \ifx\the_publ\undefined
       \ifx\the_report\undefined 
	 \errhelp{A reference must at least have a \journal \inbook \publ^^J
		  or \report field defined.}%
	 \errmessage{Unrecognised reference}%
       \else \make_report \fi
     \else \make_book \fi
   \else \make_article \fi
 \else\make_proceedings \fi
 \ifx\the_endnote\undefined\else \finalinfo\the_endnote \fi
 \amsendref
 \endgraf\endgroup
}

\def\make_report
{\paper\the_title \paperinfo\the_report\unskip \opt_pages
 \_opt\the_year{\yr\the_year}%
}
\def\make_book
{\book\the_title \opt_pages
 \_opt\the_series
 {\bookinfo\the_series
  \_opt\the_ed{\csname amsed\q_plur\the_ed\endcsname\the_ed}%
  \_opt\the_vol{\amsvol\the_vol\_opt\the_idno{\unskip, \the_idno}}%
 }%
 \amspubl\the_publ \yr\the_year \_opt\the_ISBN{\bookinfo\the_ISBN}%
}
\def\make_article
{\paper\the_title \jour\the_journal
 \_opt\the_vol{\amsvol\the_vol\_opt\the_idno{\unskip, \the_idno}}%
 \_opt\the_year{\yr\the_year}\opt_pages
}
\def\make_proceedings
{\paper\the_title \opt_pages \amsinbook\the_inbook
 \_opt\the_ed{\csname amsed\q_plur\the_ed\endcsname\the_ed}%
 \_opt\the_series{\bookinfo\the_series
   \_opt\the_vol{\amsvol\the_vol\_opt\the_idno{\unskip, \the_idno}}}%
 \_opt\the_publ{\amspubl\the_publ}\yr\the_year
}

\else % \amstexfalse

\def\_opt#1#2{\ifx#1\undefined\else{\def\__{#1\unskip}#2}\fi}
\def\opt_pages#1{\ifx\the_pages\undefined\else{\let\__\_pages#1}\fi}

\def\endref
{\iffalse{\fi}\let\par\endgraf\smallbreak\hangindent\refindent
 \setbox0=\hbox{[\the_mark\unskip]\enspace}\noindent
 \ifdim\wd0<\refindent \hbox to \refindent{\unhbox0\hfil}\else\unhbox0 \fi
 \format_author{\the_author\unskip},
 \ifx\the_inbook\undefined
   \ifx\the_journal\undefined
     \ifx\the_publ\undefined
       \ifx\the_report\undefined 
	 \errhelp{A reference must at least have a \journal \inbook \publ^^J
        	  or \report field defined.}%
         \errmessage{Unrecognised reference}%
       \else \format_report \fi
     \else \format_book \fi
   \else \format_article \fi
 \else\format_proceedings \fi
 \unskip \_opt\the_endnote{. \__}.
 \endgraf\endgroup
}

\def\format_author#1{{\rm#1}}

\def\format_report
{{\sl \the_title\unskip}, \the_report\unskip\expl_pp\opt_pages{, \__}%
 \_opt\the_year{, (\__)}}
\def\format_book
{{\sl\the_title\unskip},\expl_pp\opt_pages{ \__,}%
 \_opt\the_series{ \__\_opt\the_ed{ (\__, ed\q_plur\the_ed.)}%
 \_opt\the_vol{ \__}\_opt\the_idno{, \__},} \the_publ\unskip,
 \the_year\unskip\_opt\the_ISBN{, ISBN \__}}
\def\format_article
{``\the_title\unskip'', {\sl\the_journal\unskip\_opt\the_vol{\/ \bf\__}}%
 \_opt\the_idno{, \__}\_opt\the_year{, (\__)}\impl_pp\opt_pages{, \__}}
\def\format_proceedings
{``\the_title\unskip'',\expl_pp\opt_pages{ \__} in {\sl\the_inbook\unskip}%
 \_opt\the_ed{ (\__, ed\q_plur\the_ed.)},
 \_opt\the_series{\__\_opt\the_vol{ \__}\_opt\the_idno{, \__}, }%
 \_opt\the_publ{\__, }\the_year}

\fi % \ifamstex

\catcode`_=8 % Now underscores are for subscripts again
\catcode`@=12 % and `@' cannot be used in control sequences

